Study of electron capture rates on chromium isotopes for core-collapse simulations

Electron capture rates on \emph{fp}-shell nuclei play a pivotal role in the dynamics of stellar evolution and core collapse. These rates play a crucial role in the gravitational collapse of the core of a massive star activating the supernova explosion. As per simulation results, capture rates on chromium isotopes have a major impact on controlling the lepton-to-baryon fraction of the stellar core during the late phases of evolution of massive stars. In this paper we calculate the electron capture rates on isotopes of chromium with mass range $42\leq A \leq 65$, including neutron-deficient and neutron-rich isotopes. For the calculation of weak rates in stellar matter, we used the pn-QRPA model with separable Gamow-Teller forces and took deformation of nucleus into consideration. A recent study proved this form of pn-QRPA to be the best for calculation of GT strength distributions amongst the pn-QRPA models. The stellar weak rates are calculated over a broad range of temperature $(0.01 \times 10^{9}-30 \times 10^{9} (K))$ and density $(10-10^{11}(g/cm^{3}))$ domain. We compare our electron capture rates with the pioneering calculation of Fuller, Fowler, and Newman (FFN) and with the large-scale shell model (LSSM) calculation. Our electron capture rates are enhanced compared to the FFN and shell model rates.

==> rjp_mathdefs.tex <==
%This file contains a hopefully ever growing collection of command shortcuts and even new LaTeX commands (especially for math mode),
% that are currently in use and accepted by Romanian Journal of Physics.

%Environment and general command shortcuts
\providecommand{\beq}[1][\@empty]{\def\@ttoken{#1}\begin{equation}\dbg@ut{\@ttoken}\ifx\@empty#1 \else\label{#1}\fi}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

%Mathematical operators and various symbols
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}
\providecommand{\pd}{\ensuremath{\partial}}
\providecommand{\dd}{\ensuremath{\mathrm{d}}}
\providecommand{\id}{\ensuremath{\;\mathrm{d}}}

%bras and kets
\providecommand{\bra}[1]{\ensuremath{\left<#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right>}}
%the \braket command is thought to be the matrix element of operator #1 for state #2 (left) and state #3 (right)
\providecommand{\braket}[3]{\ensuremath{\left<#2|#1|#3\right>}}

%Commands for multiple indexes around a central token #1
%The names derive from "front up-down, back up-down" of #1 (it better be read as "left up-down, right up-down") indicating 
%the order in which indexes are passed starting with #2 (left-up or front-up). The only cool stuff about these commands is 
%that it diminishes the space between up-down left indexes and the following token.
\newcommand{\fudbud}[5]{{\!\;}^{#2}_{#3}\!\!#1^{#4}_{#5}}
\newcommand{\fubu}[3]{{\!\;}^{#2}\!\!#1^{#3}}
\newcommand{\fdbd}[3]{{\!\;}_{#2}\!\!#1_{#3}}

%put a small hat on operators!
\providecommand{\hatop}[1]{\ensuremath{\hat{\mathop{\operator@font #1}\nolimits}}}

%A small macro for generating uppercased letters of specific math font (mathfrak).
\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%


==> rrp_mathdefs.tex <==
%\newcommand{\opL}{\mathfrak{L}}
%\newcommand{\opN}{\mathfrak{N}}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

\newcommand{\ddiv}{\ensuremath{\mathop{\operator@font div}\nolimits}}
\newcommand{\grad}{\ensuremath{\mathop{\operator@font grad}\nolimits}}
\newcommand{\artanh}{\ensuremath{\mathop{\operator@font artanh}\nolimits}}
\newcommand{\sech}{\ensuremath{\mathop{\operator@font sech}\nolimits}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}

\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%

